ZipZap: A Blockchain Solution for Local Energy Trading

In the last few years, electric utility companies have increasingly invested into transactive energy systems. This trend was primarily caused by the integration of distributed energy resources (DERs) and internet-of-things (IoT) devices into their existing distribution networks. Influenced by the general interest in blockchain technologies, many industry specialists are considering new, more efficient peer-to-peer market structures for DERs. Since blockchain-based energy exchanges can automate transactions between their members and provide increased levels of security thanks to smart contracts, these new initiatives may eventually revolutionize how customers interact with utility companies. In this paper, we explore the trade-off between cost and traceability in the form of on-chain and off-chain solutions. We also propose ZipZap, a first step towards a blockchain-based local smart grid system. ZipZap is an ERC-1155 compliant solution with four different prototypes: Heavyweight, Featherweight, Lightweight and Weightless. The first three prototypes were developed in Solidity and deployed using Ethereum. Heavyweight is fully on-chain, whereas Featherweight and Lightweight showcase various levels of hybridization. Weightless, in turn, was deployed using Quorum, a gas-free alternative to Ethereum. Our evaluation uses realistic parameters and measures the impact of different types of metadata storage scopes, with some Ethereum prototypes showcasing gas cost reductions of more than 97% in comparison to our fully on-chain baseline.

==> README <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/


This package contains the IEEE Computer Society subset of the full IEEEtran
package and is intended for use with IEEE Computer Society publications.
The included version of the IEEEtran_HOWTO.pdf has been specially formatted
in IEEE Computer Society (compsoc) journal mode.


For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         conference papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for a IEEE Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf_compsoc.tex, bare_jrnl_compsoc.tex.
***************************************************************************


==> multirow/README <==
multirow.sty  2019/05/31 v2.5
bigstruts.sty  2019/05/31 v2.5
bigdelim.sty  2019/05/31 v2.5

Original Author: Jerry Leichter
Current Author:  Piet van Oostrum <piet@vanoostrum.org>

 This file may be distributed under the terms of the LaTeX Project Public
 License, as described in lppl.txt in the base LaTeX distribution.
 Either version 1.3 or, at your option, any later version.

Installation:

To generate the .sty files, run the command
   tex multirow.ins
and move the resulting .sty files to a place where LaTeX can find them, preferably
..../tex/latex/multirow

Usage:

multirow.sty:

Make an entry that will span multiple rows of a table.

\multirow[vpos]{nrows}[bigstruts]{width}[vmove]{text}

vpos is the vertical positioning: t. c. or b.

nrows is the number of rows to span.  It's up to you to leave the other
      rows empty, or the stuff created by \multirow will over-write it.
      With a positive value of nrows the spanned colomns are this row and
      (nrows-1) rows below it. With a negative value of nrows they are
      this row and (1-nrows) above it.

bigstruts is mainly used if you've used bigstrut.sty.  In that case it
      is the total number of uses of \bigstrut within the rows being
      spanned.  Count 2 uses for each \bigstrut, 1 for each \bigstrut[x]
      where x is either t or b.  The default is 0.

width is the width to which the text is to be set, or * to indicate that
      the text argument's natural width is to be used.
text is the actual text.  If the width was set explicitly, the text will
      be set in a parbox of that width; you can use \\ to force linebreaks
      where you like.

      If the width was given as * the text will be set in LR mode.  If you
      want a multiline entry in this case you should use a tabular or array
      in the text parameter.

	  If the width is given as = the width will be taken from the
	  tabular column in which it appears. This only works for p{}
	  columns and similar, for example X columns in tabularx, and LCRJ
	  columns in tabulary.

      The text is centered vertically within the range spanned by nrows,
	  unless a vpos argument is given.

vmove is a length used for fine tuning:  The text will be raised (or
      lowered, if vmove is negative) by that length above (below) wherever
       it would otherwise have gone.

For example (using both multirow and bigstrut)

\newcommand{\minitab}[2][l]{\begin{tabular}{#1}#2\end{tabular}}
\begin{tabular}{|c|c|}
\hline
\multirow{4}{1in}{Common g text} & Column g2a\\
      & Column g2b \\
      & Column g2c \\
      & Column g2d \\
\hline
\multirow{3}[6]*{Common g text} & Column g2a\bigstrut\\\cline{2-2}
      & Column g2b \bigstrut\\\cline{2-2}
      & Column g2c \bigstrut\\
\hline
\multirow{4}[8]{1in}{Common g text} & Column g2a\bigstrut\\\cline{2-2}
      & Column g2b \bigstrut\\\cline{2-2}
      & Column g2c \bigstrut\\\cline{2-2}
      & Column g2d \bigstrut\\
\hline
\multirow{4}*{\minitab[c]{Common \\ g text}} & Column g2a\\
      & Column g2b \\
      & Column g2c \\
      & Column g2d \\
\hline
\end{tabular}

If any of the spanned rows are unusually large, or if you're using
bigstrut.sty and \bigstrut's are used assymetrically about the centerline of
the spanned rows, the vertical centering may not come out right.  Use the
vmove argument in this case.

Just before "text" is expanded, the \multirowsetup macro is expanded to      
set up any special environment.  Initially, \multirowsetup contains just
\raggedright.  It can be redefined with \renewcommand.
 
bigstrut.sty:

\bigstrut[pos] where pos is t or b

    Add a bit of space above, below, or both a tabular row. The amount
	is determined by \bigstrutjot.

bigdelim.sty:

\ldelim({n}{width}[text]
\rdelim){n}{width}[text]

Put a big delimiter over n rows in a tabular, optionally preceded
(\ldelim) or followed (rdelim) by text.
	


==> multirow/multirow/README <==
multirow.sty  2019/05/31 v2.5
bigstruts.sty  2019/05/31 v2.5
bigdelim.sty  2019/05/31 v2.5

Original Author: Jerry Leichter
Current Author:  Piet van Oostrum <piet@vanoostrum.org>

 This file may be distributed under the terms of the LaTeX Project Public
 License, as described in lppl.txt in the base LaTeX distribution.
 Either version 1.3 or, at your option, any later version.

Installation:

To generate the .sty files, run the command
   tex multirow.ins
and move the resulting .sty files to a place where LaTeX can find them, preferably
..../tex/latex/multirow

Usage:

multirow.sty:

Make an entry that will span multiple rows of a table.

\multirow[vpos]{nrows}[bigstruts]{width}[vmove]{text}

vpos is the vertical positioning: t. c. or b.

nrows is the number of rows to span.  It's up to you to leave the other
      rows empty, or the stuff created by \multirow will over-write it.
      With a positive value of nrows the spanned colomns are this row and
      (nrows-1) rows below it. With a negative value of nrows they are
      this row and (1-nrows) above it.

bigstruts is mainly used if you've used bigstrut.sty.  In that case it
      is the total number of uses of \bigstrut within the rows being
      spanned.  Count 2 uses for each \bigstrut, 1 for each \bigstrut[x]
      where x is either t or b.  The default is 0.

width is the width to which the text is to be set, or * to indicate that
      the text argument's natural width is to be used.
text is the actual text.  If the width was set explicitly, the text will
      be set in a parbox of that width; you can use \\ to force linebreaks
      where you like.

      If the width was given as * the text will be set in LR mode.  If you
      want a multiline entry in this case you should use a tabular or array
      in the text parameter.

	  If the width is given as = the width will be taken from the
	  tabular column in which it appears. This only works for p{}
	  columns and similar, for example X columns in tabularx, and LCRJ
	  columns in tabulary.

      The text is centered vertically within the range spanned by nrows,
	  unless a vpos argument is given.

vmove is a length used for fine tuning:  The text will be raised (or
      lowered, if vmove is negative) by that length above (below) wherever
       it would otherwise have gone.

For example (using both multirow and bigstrut)

\newcommand{\minitab}[2][l]{\begin{tabular}{#1}#2\end{tabular}}
\begin{tabular}{|c|c|}
\hline
\multirow{4}{1in}{Common g text} & Column g2a\\
      & Column g2b \\
      & Column g2c \\
      & Column g2d \\
\hline
\multirow{3}[6]*{Common g text} & Column g2a\bigstrut\\\cline{2-2}
      & Column g2b \bigstrut\\\cline{2-2}
      & Column g2c \bigstrut\\
\hline
\multirow{4}[8]{1in}{Common g text} & Column g2a\bigstrut\\\cline{2-2}
      & Column g2b \bigstrut\\\cline{2-2}
      & Column g2c \bigstrut\\\cline{2-2}
      & Column g2d \bigstrut\\
\hline
\multirow{4}*{\minitab[c]{Common \\ g text}} & Column g2a\\
      & Column g2b \\
      & Column g2c \\
      & Column g2d \\
\hline
\end{tabular}

If any of the spanned rows are unusually large, or if you're using
bigstrut.sty and \bigstrut's are used assymetrically about the centerline of
the spanned rows, the vertical centering may not come out right.  Use the
vmove argument in this case.

Just before "text" is expanded, the \multirowsetup macro is expanded to      
set up any special environment.  Initially, \multirowsetup contains just
\raggedright.  It can be redefined with \renewcommand.
 
bigstrut.sty:

\bigstrut[pos] where pos is t or b

    Add a bit of space above, below, or both a tabular row. The amount
	is determined by \bigstrutjot.

bigdelim.sty:

\ldelim({n}{width}[text]
\rdelim){n}{width}[text]

Put a big delimiter over n rows in a tabular, optionally preceded
(\ldelim) or followed (rdelim) by text.
	

